Improving virtual host efficiency through resource and interference aware scheduling

Modern Infrastructure-as-a-Service Clouds operate in a competitive environment that caters to any user's requirements for computing resources. The sharing of the various types of resources by diverse applications poses a series of challenges in order to optimize resource utilization while avoiding performance degradation caused by application interference. In this paper, we present two scheduling methodologies enforcing consolidation techniques on multicore physical machines. Our resource-aware and interference-aware scheduling schemes aim at improving physical host efficiency while preserving the application performance by taking into account host oversubscription and the resulting workload interference. We validate our fully operational framework through a set of real-life workloads representing a wide class of modern cloud applications. The experimental results prove the efficiency of our system in optimizing resource utilization and thus energy consumption even in the presence of oversubscription. Both methodologies achieve significant reductions of the CPU time consumed, reaching up to 50%, while at the same time maintaining workload performance compared to widely used scheduling schemes under a variety of representative cloud platform scenarios.

==> discussion.tex <==
% \subsection{Algorithm performance}

% Focus on core savings metric
In order to evaluate the performance of the scheduling algorithms presented in Section \ref{sec:architecture}, we consider the amount of on-host CPU time saved
through VM consolidation over the workload performance variation (slowdown or speedup). Host CPU time can be construed as a measure of the total resource usage 
on the host, and thus lower CPU consumption relates to more efficient use of resources. Also, since most of the fraction of electricity consumed by a running server 
is proportionate to CPU utilization, lowering CPU utilization is also beneficial in terms of energy consumption. Thus, evaluating the gains in terms of efficiency
vs the performance trade-off will accurately highlight better performing schedulers in light of the main performance indicator for VM consolidation.

%Metric description
To measure scheduler performance we use:
\begin{equation*}
 M = \frac{(P_{ALG} - P_{RRS} )}{P_{RRS}} + \frac{(C_{RRS} - C_{ALG})}{C_{RRS}}
\end{equation*}
where M is the scheduler performance metric, P is the average performance of all workloads scheduled (using RRS or some other scheduling ALGorithm) and C is the
CPU time consumed by all the co-scheduled workloads when run to completion. The metric is designed to take into account the gains in performance and efficiency 
in conjunction and penalize severe performance degradation with regards to the simple round-robin scheduler.

\begin{table}
\centering
\caption{Metric evaluation of algorithms vs RRS} \label{tab:perf_metric_table}
\begin{tabular}{|c||c|c|c|c|}
 \hline
  \textbf{SR} & \textbf{RAS RS} & \textbf{IAS RS} & \textbf{RAS LS} & \textbf{IAS LS} \\
 \hline
0.5 & 0.3017322721 & 0.2569134853 & 0.3016877948 & 0.3262783336 \\
1 & 0.1645904566 & 0.2598010751 & 0.3119356019 & 0.4184069583 \\
1.5 & 0.4024503311 & 0.4777130243 & 0.285943619 & 0.3956368481 \\
2 & 0.07868456622 & 0.1507817439 & 0.2476092701 & 0.3072840804 \\
 \hline
\end{tabular}
\end{table}

\begin{figure}[t]
\centering\includegraphics[width=0.48\textwidth]{./figures/sched_metric.pdf}
\caption{Metric evaluation of RAS and IAS scheduling performance.}\label{fig:sched_metric}
% \vspace{-0.1in}
\end{figure}

% Check that in the oversubscribed case you have better performance when incorporating the interference table
% RR and Threshold algorithms should be better in terms of raw performance ONLY on the under-subscribed, heavy-load scenario
With regards to the experimental results presented in the previous chapter, we can conclude that both RAS and IAS
outperform round-robin placement of VMs on the compute host in terms of resource consumption and, in the over-subscribed cases, in performance as well. 
Considering our composite metric, with results depicted in Table \ref{tab:perf_metric_table} and Figure \ref{fig:sched_metric} for graphic comparison, the performance
of both schedulers peaks for $SR$ around $1$-$1.5$, i.e. when the server is conservatively oversubscribed. IAS seems to significantly outperform 
RAS in all cases, except for $SR=0.5$ in the random scenario. The schedulers' performance is minimum for $SR=2$ as in that case there are few things they can do 
in order to improve performance and reduce core hours consumption other than consolidate idle workloads. Whatever the pinning is, for $SR=2$, the performance degradation
that workloads suffer is severe. 

%Irrelevant with new metric

%Considering our composite metric, with results depicted in Table \ref{tab:perf_metric_table} and Figure \ref{fig:sched_metric} for graphic comparison, the performance of 
%TBS seems to peak in the under-subscribed to lightly over-subscribed case in both random and latency-critical scenarios (RS and LS respectively). Interference-based scheduling 
%seems to significantly outperform TBS in the over-subscribed case, especially in the non-latency critical case. This is to be expected, as latency-critical workloads usually 
%suffer less from interference from different workloads than from similar workloads. Therefore, as the interference scheduler has few good candidates to co-schedule with the 
%latency-critical workloads, the results of consolidation are worse compared with the random scenario. Still, even in this case, interference-aware scheduling easily outperforms 
%the threshold-based scheduler.

% Aggressiveness of dynamic VM placement (Threshold vs Interference)
In terms of aggressiveness, RAS is more tunable than IAS, due to the threshold parameter being used to consolidate VMs. Although the 120\% setting 
used in our experiments limits RAS, it is selected in order to provide the best results of this scheduler class given our experimental setup. IAS seems
more aggressive in our results but this is an artifact of the workload selection (or not, in the random scenario). Depending on the best way to avoid workload 
interference then, IAS can vary the intensity of VM consolidation.

% Is RR state-of-the-art? Is IBS the next best thing?


